CaBaGe: Data-Free Model Extraction using ClAss BAlanced Generator Ensemble

Machine Learning as a Service (MLaaS) is often provided as a pay-per-query, black-box system to clients. Such a black-box approach not only hinders open replication, validation, and interpretation of model results, but also makes it harder for white-hat researchers to identify vulnerabilities in the MLaaS systems. Model extraction is a promising technique to address these challenges by reverse-engineering black-box models. Since training data is typically unavailable for MLaaS models, this paper focuses on the realistic version of it: data-free model extraction. We propose a data-free model extraction approach, CaBaGe, to achieve higher model extraction accuracy with a small number of queries. Our innovations include (1) a novel experience replay for focusing on difficult training samples; (2) an ensemble of generators for steadily producing diverse synthetic data; and (3) a selective filtering process for querying the victim model with harder, more balanced samples. In addition, we create a more realistic setting, for the first time, where the attacker has no knowledge of the number of classes in the victim training data, and create a solution to learn the number of classes on the fly. Our evaluation shows that CaBaGe outperforms existing techniques on seven datasets -- MNIST, FMNIST, SVHN, CIFAR-10, CIFAR-100, ImageNet-subset, and Tiny ImageNet -- with an accuracy improvement of the extracted models by up to 43.13%. Furthermore, the number of queries required to extract a clone model matching the final accuracy of prior work is reduced by up to 75.7%.

==> Tables/CIFAR_Scaling.tex <==
\begin{table}
% Dataset Model Teacher IDEAL DGP1x 2x 4x 8x 16x 32x
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|}
\toprule
Dataset & Model & Teacher & IDEAL & \ours 1xQB & 2xQB & 4xQB & 8xQB & 16xQB & 32xQB\\
\midrule
CIFAR-10 & AlexNet & 84.76 & 65.61 & 47.97 & 55.10 & 63.15 & \textbf{70.46} & 72.08 & 75.54 \\
\midrule
CIFAR-10 & ResNet34 & 93.45 & 68.82 & 20.64 & 38.46 & \textbf{70.51} & 80.55 & 88.02 & 90.83 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/DGP_novelty_timecomparison.tex <==
\begin{table*}
    \centering
    \footnotesize
    \begin{tabular}{l|l r@{}l r@{}ll r@{}ll r@{}ll}
    \toprule
    \textbf{Dataset} & \textbf{Model} & \multicolumn{2}{c}{\textbf{\ours no SQ+GE}} & \multicolumn{3}{c}{\textbf{\ours no SQ}} & \multicolumn{3}{c}{\textbf{\ours no GE}} & \multicolumn{3}{c}{\textbf{\ours}} \\
    \midrule
MNIST & MLP & $1.34$&$\pm0.82$ & $0.90$&$\pm0.36$&(-, $p$=0.309) & $1.48$&$\pm0.74$&(+, $p$=0.788) & $1.04$&$\pm0.21$&(-, $p$=0.462) \\
& LeNet & $1.01$&$\pm0.76$ & $1.42$&$\pm0.67$&(+, $p$=0.389) & $1.58$&$\pm0.78$&(+, $p$=0.269) & $1.70$&$\pm0.37$&(+, $p$=0.102) \\
& AlexNet & $2.07$&$\pm1.04$ & $2.55$&$\pm0.64$&(+, $p$=0.407) & $2.20$&$\pm0.83$&(+, $p$=0.824) & $2.04$&$\pm0.14$&(-, $p$=0.967) \\

\midrule
FMNIST & MLP & $12.23$&$\pm6.42$ & $11.02$&$\pm3.31$&(-, $p$=0.721) & $8.23$&$\pm3.54$&(-, $p$=0.258) & $8.42$&$\pm0.56$&(-, $p$=0.234) \\
& LeNet & $13.68$&$\pm7.10$ & $11.25$&$\pm4.33$&(-, $p$=0.536) & $10.22$&$\pm3.45$&(-, $p$=0.361) & $12.31$&$\pm0.33$&(-, $p$=0.688) \\
& AlexNet & $14.70$&$\pm7.25$ & $13.15$&$\pm5.16$&(-, $p$=0.711) & $14.62$&$\pm4.70$&(-, $p$=0.986) & $13.25$&$\pm0.35$&(-, $p$=0.676) \\

\midrule
SVHN & VGG-16 & $13.39$&$\pm2.93$ & \color{blue}{$18.06$}&$\pm1.86$&(+, $p$=0.011) & \color{blue}{$19.40$}&$\pm4.57$&(+, $p$=0.031) & \color{blue}{$22.64$}&$\pm0.54$&(+, $p$=0.000) \\
& ResNet-18 & $15.80$&$\pm2.66$ & \color{blue}{$21.25$}&$\pm0.36$&(+, $p$=0.002) & \color{blue}{$20.51$}&$\pm0.79$&(+, $p$=0.005) & \color{blue}{$22.51$}&$\pm0.19$&(+, $p$=0.001) \\
& AlexNet & $11.55$&$\pm5.43$ & $10.23$&$\pm5.05$&(-, $p$=0.704) & \color{red}{$3.82$}&$\pm0.83$&(-, $p$=0.015) & $10.54$&$\pm2.02$&(-, $p$=0.714) \\

\midrule
CIFAR-10 & AlexNet & $35.70$&$\pm12.48$ & $35.36$&$\pm14.86$&(-, $p$=0.970) & $25.95$&$\pm12.98$&(-, $p$=0.266) & \color{red}{$19.06$}&$\pm10.22$&(-, $p$=0.040) \\
& ResNet-34 & $74.08$&$\pm10.64$ & \color{blue}{$95.94$}&$\pm0.30$&(+, $p$=0.002) & $85.04$&$\pm9.31$&(+, $p$=0.114) & \color{blue}{$103.09$}&$\pm2.20$&(+, $p$=0.000) \\

\midrule
ImageNet$_{12}$ & AlexNet & $8.23$&$\pm1.14$ & \color{blue}{$12.19$}&$\pm0.92$&(+, $p$=0.000) & \color{blue}{$10.62$}&$\pm1.34$&(+, $p$=0.009) & \color{blue}{$13.29$}&$\pm2.40$&(+, $p$=0.002) \\
& VGG-16 & $77.89$&$\pm10.92$ & \color{blue}{$93.14$}&$\pm9.25$&(+, $p$=0.035) & $87.51$&$\pm10.42$&(+, $p$=0.189) & $73.79$&$\pm0.05$&(-, $p$=0.437) \\

    \bottomrule
    \end{tabular}
    \caption{\textbf{Time taken} in minutes of \ours and the ablation settings shown along with 95\% confidence interval.  Along with the Time, we use column \textbf{\ours no SQ+GE} as baseline, and compare all other columns' result with the baseline, using independent t-test. Statistically significant result are colored. Blue indicates improvements, and red indicates deterioration.}
    \label{tab:novl_eval_time_compare}
    \end{table*}

==> Tables/IDEAL_reproduce_comparison.tex <==

\begin{table}
\centering
\caption{Accuracy (\%) of student models trained with various teacher models for comparison between IDEAL, IDEAL reproduced, DGP}
% \label{tab:accuracy}
\begin{tabular}{|l|l|c|c|c|c|c|}
\toprule
Dataset & Model & Teacher & IDEAL & Ideal Reproduced & \ours 1xQuery & \ours 2xQuery \\
\midrule
\multirow{3}{*}{MNIST} & MLP & 98.25 & \textbf{88.41} & 18.5 & 58.04$\pm$3.06 & 70.37$\pm$4.97 \\
& LeNet & 99.27 & \textbf{96.32} & 93.7 & 94.12$\pm$0.58 & 95.82$\pm$1.19 \\
& AlexNet & 99.35 & {96.51} & 82.7 & 94.52$\pm$0.80 & \textbf{97.95$\pm$0.20} \\
\midrule
\multirow{3}{*}{FMNIST} & MLP & 84.54 & 76.95 & 19.0 & 78.63$\pm$1.60 & \textbf{80.08$\pm$1.88} \\
& LeNet & 90.23 & \textbf{83.92} & 27.8 & 68.36$\pm$2.04 & 75.80$\pm$1.84 \\
& AlexNet & 92.66 & \textbf{86.14} & 35.20 & 80.13$\pm$1.90 & 84.67$\pm$1.17 \\
\midrule
\multirow{3}{*}{SVHN} & AlexNet & 89.82 & \textbf{84.42} & 67.2 & 78.39$\pm$2.68 & 81.10$\pm$1.21 \\
& VGG-16 & 94.41 & 86.91 & 76.7 & 86.25$\pm$1.04 & \textbf{89.67$\pm$0.42} \\
& ResNet-18 & 95.28 & \textbf{87.65} & 63.9 & 82.42$\pm$2.41 & 83.58$\pm$2.25 \\
\midrule
\multirow{2}{*}{CIFAR-10} & AlexNet & 84.76 & {65.61} & - & 47.97 & 55.10 (75.4 for 32xQB)\\
& ResNet-34 & 93.85 & {68.82} & - & 31.37 & 50.51 (90.77 for 32xQB) \\
\midrule
\multirow{2}{*}{ImageNet Subset} & AlexNet & 72.96 & \textbf{53.72} & - & 47.94$\pm$3.22 & 49.77$\pm$4.14 \\
& VGG-16 & 78.53 & \textbf{57.95} & - & 30.42$\pm$3.68 & 40.93$\pm$3.10 \\
\midrule
\multirow{2}{*}{CIFAR100} & AlexNet & 66.24 & 23.85 & - & - & tbd \\
& ResNet-34 & 89.45 & 36.96 & - & \textbf{42.42} & 56.93 \\
\midrule
\multirow{2}{*}{tinyImageNet} & VGG-16 & 52.96 & 21.72 & - & - & tbd \\
& ResNet-34 & 64.53/58 & 27.95 & - & - & \textbf{33.03} \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/ablation_generator_ensemble_size.tex <==
\begin{table}
\centering
\footnotesize
\begin{tabular}{ r|rrrrr  }
 \toprule
Setting & 1  &  2 & 4 & 8 & 16 \\ \midrule
CIFAR100 SL & 69.47 $\pm$ 0.88 & 69.66 &70.28 & 71.33 & 70.9 $\pm$ 1.84 \\
CIFAR100 HL  & 60.69 & 61.69 & 62.52 & 63.25 & 62.91 \\
 \bottomrule
\end{tabular}
\caption{Impact of generator ensemble size. \todo{Consider having plot instead of table}
}
\label{tab:gen-ensemble-size}
\end{table}

==> Tables/ideal_table.tex <==

\begin{table*}
\centering
\caption{Accuracy (\%) of student models for IDEAL, Reproduced, and Ideal fixed. Results are averaged over 2 runs. Random seed is set, so most of the runs should have the same/similar result}
\begin{tabular}{|l|l|c|c|c|c|}
\toprule
Dataset & Model & IDEAL & Reproduced & Ideal fixed & \ours 2xQuery \\
\midrule
\multirow{3}{*}{MNIST} & MLP & 88.41 & 32.20 & 14.00 & 70.37$\pm$4.97 \\
& LeNet & 96.32 & 95.20 & 86.40 & 95.82$\pm$1.19 \\
& AlexNet & 96.51 & 95.40 & 66.30 & 97.95$\pm$0.20 \\
\midrule
\multirow{3}{*}{FMNIST} & MLP & 76.95 & 38.9 & 19.00 & 80.08$\pm$1.88 \\
& LeNet & 83.92 & 84.50 & 27.80 & 75.80$\pm$1.84 \\
& AlexNet & 86.14 & 83.60 & 35.20 & 84.67$\pm$1.17 \\
\midrule
\multirow{3}{*}{SVHN} & AlexNet & 84.42 & 81.70 & 67.00 & 81.10$\pm$1.21 \\
& VGG-16 & 86.91 & 88.85±0.35 & 68.35±7.00 & 89.67$\pm$0.42 \\
& ResNet-18 & 87.65 & 84.7 & 72.60 & 83.58$\pm$2.25 \\
\midrule
\multirow{2}{*}{CIFAR-10} & AlexNet & 65.61 & 66.80 & 25.50 & 41.05 $\pm$ 2.15 (32xQB: 83.57 $\pm$ 0.08) \\
& ResNet-34 & 68.82 & - & 20.40 & 34.77 $\pm$ 3.60 (32xQB: 90.42 $\pm$ 0.30) \\
\midrule
\multirow{2}{*}{ImageNet susnet} & AlexNet & 53.72 & - & - & 49.77$\pm$4.14 \\
& VGG-16 & 57.95 & - & - & 40.93$\pm$3.10 \\
\midrule
\multirow{2}{*}{CIFAR100} & AlexNet & 23.85 & - & - & tbd \\
& ResNet-34 & 36.96 & - & - & 56.93 \\
\midrule
\multirow{2}{*}{Tiny ImageNet} & VGG-16 & 21.72 & - & - & tbd \\
& ResNet-34 & 27.95 & - & - & 33.03 \\
\bottomrule
\end{tabular}
\end{table*}


==> Tables/ideal_teachers.tex <==
\begin{table}
\centering
\caption{Teacher accuracy (\%) for IDEAL, Reproduced, and Ideal Fixed.}
\begin{tabular}{|l|l|c|c|c|}
\toprule
Dataset & Model & Teacher (IDEAL) & Teacher (Reproduced) & Teacher (Fixed) \\
\midrule
\multirow{3}{*}{MNIST} & MLP & 98.25 & 96.20 & 98.2 \\
& LeNet & 99.27 & 99.2 & - \\
& AlexNet & 99.35 & 99.1 & - \\
\midrule
\multirow{3}{*}{FMNIST} & MLP & 84.54 & 84.0 & - \\
& LeNet & 90.23 & 90.2 & - \\
& AlexNet & 92.66 & 91.1 & - \\
\midrule
\multirow{3}{*}{SVHN} & AlexNet & 89.82 & 89.00 & - \\
& VGG-16 & 94.41 & 94.20 & - \\
& ResNet-18 & 95.28 & 91.0 & - \\
\midrule
\multirow{2}{*}{CIFAR-10} & AlexNet & 84.76 & - & 84.76 \\
& ResNet-34 & 93.85 &  - & 93.45 \\
\midrule
\multirow{2}{*}{ImageNet subset} & AlexNet & 72.96 & - & - \\
& VGG-16 & 78.53 & - & - \\
\midrule
\multirow{2}{*}{CIFAR100} & AlexNet & 66.24 & - & - \\
& ResNet-34 & 89.45 & - & - \\
\midrule
\multirow{2}{*}{Tiny ImageNet} & VGG-16 & 52.96 & - & - \\
& ResNet-34 & 64.53 & 58 & - \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/query_limited_fidelity.tex <==
\begin{table*}[ht]
    \centering
    \caption{Fidelity (\%) of \clone models trained with various teacher models on MNIST, FMNIST, SVHN, CIFAR10, and ImageNet subset in the \textbf{query-limited} setting. Best results are in bold. IDEAL$^*$ is the reproduced result after fixing an error in the original repo's code.}
    \label{tab:qblimited_accuracy2}
    \begin{tabular}{l|l|c c c c c}
    \toprule
    \textbf{Dataset} & \textbf{Model} & \textbf{Teacher} & \textbf{IDEAL} & \textbf{DisGUIDE} & \textbf{DGP} \\
    \midrule
MNIST & MLP & - & - & $13.23\pm2.59$ & \boldsymbol{$54.08\pm4.93$} \\& LeNet & - & - & $87.65\pm2.07$ & \boldsymbol{$95.66\pm0.57$} \\& AlexNet & - & - & $18.83\pm5.93$ & \boldsymbol{$86.88\pm1.25$} \\
\midrule
FMNIST & MLP & - & - & $41.60\pm0.33$ & \boldsymbol{$83.00\pm5.63$} \\& LeNet & - & - & $61.47\pm3.21$ & \boldsymbol{$70.01\pm0.85$} \\& AlexNet & - & - & $54.46\pm5.90$ & \boldsymbol{$82.98\pm0.65$} \\
\midrule
SVHN & VGG-16 & - & - & $84.80\pm0.60$ & \boldsymbol{$83.30\pm3.06$} \\& ResNet-18 & - & - & $79.75\pm2.11$ & \boldsymbol{$81.01\pm0.30$} \\& AlexNet & - & - & $23.60\pm5.96$ & \boldsymbol{$77.45\pm2.68$} \\
\midrule
CIFAR-10 & AlexNet & - & - & $24.27\pm1.23$ & \boldsymbol{$36.41\pm1.62$} \\& ResNet-34 & - & - & $21.81\pm7.14$ & \boldsymbol{$26.11\pm2.70$} \\
\midrule
CIFAR-100 & AlexNet & - & - & $27.11\pm0.41$ & \- \\& ResNet-34 & - & - & $33.71\pm0.98$ & \boldsymbol{$46.78\pm1.93$} \\
\midrule
ImageNet$_{12}$ & AlexNet & - & - & $21.73\pm2.11$ & \boldsymbol{$51.91\pm3.66$} \\& VGG-16 & - & - & $32.92\pm2.55$ & \boldsymbol{$36.58\pm13.02$} \\
\midrule
tinyImageNet & ResNet-34 & - & - & $13.04\pm3.16$ & \- \\& VGG-16 & - & - & $9.37\pm1.86$ & \boldsymbol{$14.84\pm0.64$} \\

    \bottomrule
    \end{tabular}
    \end{table*}

==> Tables/query_unlimited.tex <==

\begin{table}[h]
\centering
\caption{Accuracy (\%) of student models trained with various teacher models on various datasets with different query budget. Best results are in bold. Best results of the baselines are underlined. “Improvement” denotes the improvements of IDEAL compared with the best baseline.}
\begin{tabular}{|l|l|c|c|c|c|c|}
\toprule
Dataset & Model & Teacher & DisGUIDE & Ideal fixed & \ours 1xQuery \\
\midrule
\multirow{3}{*}{MNIST} & MLP & 98.25 & - & 14.00 & 58.04$\pm$3.06 \\
& LeNet & 99.27 & - & 86.40 & 94.12$\pm$0.58 \\
& AlexNet & 99.35 & - & 66.30 & 94.52$\pm$0.80 \\
\midrule
\multirow{3}{*}{FMNIST} & MLP & 84.54 & - & 19.00 & 78.63$\pm$1.60 \\
& LeNet & 90.23 & - & 27.80 & 68.36$\pm$2.04 \\
& AlexNet & 92.66 & - & 35.20 & 80.13$\pm$1.90 \\
\midrule
\multirow{3}{*}{SVHN} & AlexNet & 89.82 & - & 67.00 & 78.39$\pm$2.68 \\
& VGG-16 & 94.41 & - & 68.35±7.00 & 86.25$\pm$1.04 \\
& ResNet-18 & 95.28 & - & 72.60 & 82.42$\pm$2.41 \\
\midrule
\multirow{2}{*}{CIFAR-10} & AlexNet & 84.76 & - & 25.50 & 33.48 $\pm$ 3.04 \\
& ResNet-34 & 93.85 & - & 20.40 & 22.27 $\pm$ 1.15 \\
\midrule
\multirow{2}{*}{ImageNet subnet} & AlexNet & 72.96 & - & - & 47.94$\pm$3.22 \\
& VGG-16 & 78.53 & - & - & 30.42$\pm$3.68 \\
\midrule
\multirow{2}{*}{CIFAR100} & AlexNet & 66.24 & - & - & - \\
& ResNet-34 & 89.45 & - & - & 42.42 \\
\midrule
\multirow{2}{*}{tinyImageNet} & VGG-16 & 52.96 & - & - & - \\
& ResNet-34 & 64.53/58 & - & - & - \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/replay_comparison.tex <==
\begin{table}[ht]
\centering
\caption{Accuracy (\%) after dropping 1-classic-12}
\label{tab:accuracy_dropped_1-classic-12}
\begin{tabular}{|l|l|c||c|c||c|c|}
\toprule
Dataset & Model & Teacher & DisGUIDE & DisGUIDE$^*$ & \ours no DWBR & \ours \\
\midrule
\multirow{3}{*}{MNIST} & MLP & 98.25 & $12.57 \pm 2.12$ & $19.02\pm5.33$ & $21.02\pm5.33$ & \textcolor{blue}{$58.04 \pm 3.06$} \\
 & LeNet & 99.27 & $90.59 \pm 0.85$ & $91.44\pm1.50$ & $95.63\pm0.72$ & \textcolor{red}{$94.12 \pm 0.58$} \\
 & AlexNet & 99.35 & $28.36 \pm 5.37$ & $23.71\pm5.13$ & $81.09\pm0.75$ & \textcolor{blue}{$94.52 \pm 0.80$} \\
\midrule
\multirow{3}{*}{FMNIST} & MLP & 84.54 & $41.80 \pm 4.27$ & $51.89\pm7.49$ & $46.84\pm2.47$ & \textcolor{blue}{$78.63 \pm 1.60$} \\
 & LeNet & 90.23 & $62.14 \pm 1.44$ & \textcolor{red}{$59.76\pm0.41$} & $72.26\pm1.40$ & $68.36 \pm 2.04$ \\
 & AlexNet & 92.66 & $54.23 \pm 1.19$ & $58.49\pm3.67$ & $79.34\pm1.30$ & $80.13 \pm 1.90$ \\
\midrule
\multirow{3}{*}{SVHN} & AlexNet & 89.82 & $18.13 \pm 3.09$ & $23.87\pm6.91$ & $63.71\pm3.86$ & \textcolor{blue}{$78.39 \pm 2.68$} \\
 & VGG-16 & 94.41 & $13.91 \pm 4.01$ & \textcolor{blue}{$65.45\pm4.96$} & $89.43\pm0.54$ & \textcolor{red}{$86.25 \pm 1.04$} \\
 & ResNet-18 & 95.28 & $56.42 \pm29.06$ & \textcolor{blue}{$77.69\pm0.62$} & $77.95\pm1.24$ & $82.42 \pm 2.41$ \\
\midrule
\multirow{2}{*}{CIFAR10} & AlexNet & 84.76 & $20.60 \pm 1.52$ & \textcolor{blue}{$25.96\pm1.30$} & $32.84\pm0.54$ & $33.48 \pm 3.04$ \\
 & ResNet-34 & 93.85 & $23.85 \pm 3.59$ & $21.18\pm1.85$ & $29.97\pm0.49$ & \textcolor{red}{$22.27 \pm 1.15$} \\
\midrule
\multirow{2}{*}{ImageNet12} & AlexNet & 72.96 & $43.86 \pm 1.30$ & \textcolor{red}{$26.57\pm1.53$} & $47.19\pm3.98$ & \textcolor{blue}{$51.34 \pm 1.64$} \\
 & VGG-16 & 78.53 & $43.28 \pm 7.90$ & $36.79\pm5.35$ & $52.83\pm6.53$ & \textcolor{red}{$40.40 \pm 2.07$} \\
\bottomrule
\end{tabular}
\end{table}
\clearpage

\begin{table*}[ht]
\centering
\caption{Accuracy (\%) after dropping 1-WRBR-3}
\label{tab:accuracy_dropped_1-WRBR-3}
\begin{tabular}{|l|l|c||c|c|c|c|}
\toprule
Dataset & Model & Teacher & DisGUIDE & DisGUIDE$^*$ & \ours no DWBR & \ours \\
\midrule
\multirow{3}{*}{MNIST} & MLP & 98.25 & $12.57 \pm 2.12$ & \textcolor{red}{$11.35\pm0.00$} & $21.02\pm5.33$ & \textcolor{blue}{$58.04 \pm 3.06$} \\
 & LeNet & 99.27 & $90.59 \pm 0.85$ & \textcolor{blue}{$94.34\pm1.10$} & $95.63\pm0.72$ & \textcolor{red}{$94.12 \pm 0.58$} \\
 & AlexNet & 99.35 & $28.36 \pm 5.37$ & \textcolor{blue}{$75.36\pm2.49$} & \textcolor{blue}{$81.09\pm0.75$} & \textcolor{blue}{$94.52 \pm 0.80$} \\
\midrule
\multirow{3}{*}{FMNIST} & MLP & 84.54 & $41.80 \pm 4.27$ & $43.81\pm3.48$ & $46.84\pm2.47$ & \textcolor{blue}{$78.63 \pm 1.60$} \\
 & LeNet & 90.23 & $62.14 \pm 1.44$ & \textcolor{blue}{$69.07\pm0.97$} & \textcolor{blue}{$72.26\pm1.40$} & $68.36 \pm 2.04$ \\
 & AlexNet & 92.66 & $54.23 \pm 1.19$ & \textcolor{blue}{$75.21\pm1.43$} & \textcolor{blue}{$79.34\pm1.30$} & $80.13 \pm 1.90$ \\
\midrule
\multirow{3}{*}{SVHN} & AlexNet & 89.82 & $18.13 \pm 3.09$ & \textcolor{blue}{$63.26\pm1.43$} & $63.71\pm3.86$ & \textcolor{blue}{$78.39 \pm 2.68$} \\
 & VGG-16 & 94.41 & $13.91 \pm 4.01$ & \textcolor{blue}{$88.20\pm1.18$} & \textcolor{blue}{$89.43\pm0.54$} & \textcolor{red}{$86.25 \pm 1.04$} \\
 & ResNet-18 & 95.28 & $56.42 \pm29.06$ & \textcolor{blue}{$77.36\pm3.35$} & $77.95\pm1.24$ & $82.42 \pm 2.41$ \\
\midrule
\multirow{2}{*}{CIFAR10} & AlexNet & 84.76 & $20.60 \pm 1.52$ & $21.83\pm0.84$ & \textcolor{blue}{$32.84\pm0.54$} & $33.48 \pm 3.04$ \\
 & ResNet-34 & 93.85 & $23.85 \pm 3.59$ & $25.52\pm2.67$ & \textcolor{blue}{$29.97\pm0.49$} & \textcolor{red}{$22.27 \pm 1.15$} \\
\midrule
\multirow{2}{*}{ImageNet12} & AlexNet & 72.96 & $43.86 \pm 1.30$ & $43.17\pm1.18$ & $47.19\pm3.98$ & \textcolor{blue}{$51.34 \pm 1.64$} \\
 & VGG-16 & 78.53 & $43.28 \pm 7.90$ & $35.95\pm7.06$ & \textcolor{blue}{$52.83\pm6.53$} & \textcolor{red}{$40.40 \pm 2.07$} \\

\bottomrule
\end{tabular}
\end{table*}

